Geometry-Aware Recurrent Neural Networks for Active Visual Recognition

We present recurrent geometry-aware neural networks that integrate visual information across multiple views of a scene into 3D latent feature tensors, while maintaining an one-to-one mapping between 3D physical locations in the world scene and latent feature locations. Object detection, object segmentation, and 3D reconstruction is then carried out directly using the constructed 3D feature memory, as opposed to any of the input 2D images. The proposed models are equipped with differentiable egomotion-aware feature warping and (learned) depth-aware unprojection operations to achieve geometrically consistent mapping between the features in the input frame and the constructed latent model of the scene. We empirically show the proposed model generalizes much better than geometryunaware LSTM/GRU networks, especially under the presence of multiple objects and cross-object occlusions. Combined with active view selection policies, our model learns to select informative viewpoints to integrate information from by "undoing" cross-object occlusions, seamlessly combining geometry with learning from experience.

==> abstract_old.tex <==
\begin{abstract}

Cross-object occlusions remain an important source of failures for current state-of-the-art object detectors. Actively selecting camera views for ``undoing"  occlusions and recovering missing information has been identified as an important field of research since as early as 1980's, under the name {\it active vision}. Yet, 1980's active vision was not equipped with deep neural detectors, memory modules, or view selection policies, and often attempted tasks and imagery that would appear elementary with current detectors, even from a single camera view. On the other hand, the recent resurrection of active vision \cite{} has focused on reconstructing or classifying isolated objects. This work presents a paradigm for active object recognition under heavy occlusions, as was the original premise. 

It introduces a geometry-aware 3D neural memory that accumulates information of the full scene across multiple camera views into a 3D feature tensor in a geometrically consistent manner: information regarding the same 3D physical point is placed nearby in the tensor using egomotion-aware feature warping and (learned) depth-aware unprojection operations. Object detection, segmentation, and 3D reconstruction is then carried out directly using the accumulated 3D feature memory. The proposed model does not need to commit early to object detections, as current geometry-unaware object detection in 2D videos, and generalizes much better than geometry-unaware LSTM/GRU memories. The lack of geometric constraints on previous architectures appears to be the bottleneck for handling combinatorial explosions of visual data due to cross-object occlusions. The proposed model handles heavy occlusions even when trained with very little training data, by moving the head of the active observer between nearby views, seamlessly combining geometry with learning from experience.

%The proposed visual memory 
%Current paradigms of object detections in videos proceed by detecting objects at every frame using robust SOTA static image architecture at each frame, and smooth  their results in time \cite{}. Deep neural memory modules such as 2dconv lstms or GRUs have shown to often overfit \cite{} to the visual input. Both static object detectors and feature memories fail at occlusions, when objects are closeby.  We propose a visual memory
%2d memory modules, like LSTMs or GRUs,  
%We propose an architecture for detecting, segmenting and 3d reconstructing objects under clutter 

 \end{abstract}
 %\todo{mention pointnet}

==> expnew_old.tex <==
\section{Experiments} \label{sec:experiments}

%\paragraph{Datasets and experimental settings}
We test our models in two types of simulated environments: i)  scenes we create using synthetic 3D object models from  ShapeNet~\cite{shapenet2015}.  The generated scenes contain  single or multiple objects on a table surface. ii) scenes from the SUNCG~\cite{song2016ssc} dataset, sampled around an object of interest. Each 3D scene is rendered from a viewing sphere which has $3\times18$ possible views with 3 camera elevations $(20^{\circ}, 40^{\circ}, 60^{\circ})$ and 18 azimuths $(0^{\circ}, 20^{\circ}, \dots, 340^{\circ})$. The agent is allowed to move to one of the 8 adjacent views at every time step.
 %We consider the viewing angles available in the dataset \todo{???}. 
%For each scene, 
%We create a simulated environment where the camera is able to move around, by rendering
  We voxelize each 3D scene at a resolution of $64\times 64\times 64$. 
  %We also show results of multi-view reconstruction of single objects on scenes sampled from SUNCG~\cite{song2016ssc} dataset.
 % \iffalse For experiments with active vision, we pretrain the model with random input views first. We then freeze the rest of the model while training the active vision policy. \todo{ziyan please check for correctness}.\fi 
  
  We pretrain our geometry-aware recurrent neural network using randomly selected view sequences so that it does not overfit to the biases of the view selection policy. 
  %For training details, we first train the visual memory using random view sequences, so that it does not overfit to the biases of the view selection policy. 
  We then train our view selection policy while the weights of the recurrent neural network are kept fixed. 


%For each time step $t$, the agent is allowed to move to its 8-connected adjacent views. For single object, we choose three popular categories: chair, car, airplane and applying the train/val/test split according to ~\cite{shapenet2015}'s settings. 

%The single object dataset consists of xxx chairs, xxx cars, and xxx mugs.

%The multiobject dataset consists of ...

%\todo{this section is a mess: all of info about the datasets is down below instead of in this paragraph}

%\paragraph{Evaluation Metrics}

%For 3D reconstruction, we use mean IoU between groundtruth 3D voxel occupancy and 3D predicted voxel occupancy. For segmentation, we compute the mean IoU of all objects in a scene.

\paragraph{Multi-view reconstruction of single objects}
We compare the performance of the geometry-aware recurrent network against alternatives on the task of 3D reconstruction of single objects using  \textit{randomly selected} camera views (no active vision). We consider three object categories from ShapeNet: chairs, cars, and airplanes. We split the data into training, validation, and test according to ~\cite{shapenet2015}. We train a single 3d reconstruction model for all categories using supervision from groundtruth 3D voxel occupancy. We compare the proposed geometry-aware recurrent net \textit{ours} against the following baselines: 
\begin{enumerate}
    \item \textit{1D-LSTM}: an  LSTM network, similar to the one used in \cite{DBLP:journals/corr/abs-1711-03129,DBLP:journals/corr/abs-1709-00507}. In each frame, given RGB and depth as input, it produces through a 2D convolutional encoder a feature embedding vector by flattening the last 2D convolutional feature map. The embedding vector is fed into a (fully-connected) LSTM layer and the output of the LSTM is decoded into a 3D occupancy grid through a series of 3D convolutions. We detail its architecture in the Appendix. 
    \item  Learnt Stereo Machines (\textit{LSM}) of \cite{LSM}. This model aggregates information using a 3D GRU layer, similar to ours, by unprojecting convolutional features extracted from RGB images using \textit{absolute} groundtruth camera poses. Absolute pose may be hard to obtain  and it may not be meaningful in the presence of multiple objects,  our method only requires relative pose. They use a late unprojection as opposed to our proposed early depth-aware unprojection. We use the publicly available code of ~\cite{LSM} and retrain their model for our setup.
    \item \textit{LSMdepth}. An LSM alternative that uses depth as an additional input channel  and performs late unprojection on features extracted from the concatenation of depth and RGB.
\end{enumerate}
%(i)  (\textit{2D LSTM}).  (ii) Learnt Stereo Machines (\textit{LSM}) of \cite{LSM}.  (iii) An LSM alternative that uses depth as an additional input channel (\textit{LSMdepth}), and performs late unprojection on features extracted from the concatenation of depth and RGB. 
All methods are trained and tested on sequences of randomly selected nearby camera views. 


We report Intersection over Union (IoU) between the predicted and groundtruth occupancy grids in each of four camera views for our model and baselines in the test set in Table ~\ref{tab:IoU_single_multi}. More visualization results are included in the supplementary material. The proposed geometry-aware recurrent neural network outperforms the baselines. The LSM outperforms our  method on the first input view. However, after aggregating  information from more views, our method consistently outperforms all alternatives.

For SUNCG, we similarly test our proposed model on 3D reconstruction of  (usually single) objects using randomly selected camera views as input.  Intersection over Union (IoU) between the predicted and groundtruth voxel occupancy grids in each of four consecutive camera views for our model and LSTM baseline  are shown in Table~\ref{tab:IoU_single_suncg}.  Qualitative results are included in the Appendix. 

%Table~\ref{tab:single_obj}.
%As we can see, our methods that aggregating on 3D features outperforms method that aggregate on 2D features as 3D features stores semantic information spatially in a geometric consistent manner. The difference between our method and LSM is that we directly unproject on depth instead of a semantic map ectracted from RGB image. 
%\begin{table}[t!]
%\centering
%\begin{tabular}{c|cccccccc}
%                  & \multicolumn{4}{c}{single object}                      & \multicolumn{4}{c}{multi-objects} \\ \cline{2-9} 
%                  & view-1 & view-2 & view-3 & \multicolumn{1}{c|}{view-4} & view-1 & view-2 & view-3 & view-4 \\ \hline
%2D LSTM           & 0.57   & 0.59   & 0.60   & \multicolumn{1}{c|}{0.60}   & %0.11   & 0.15   & 0.17   & 0.20   \\
%GVM+gt depth     & 0.55   & \textbf{0.69}   & \textbf{0.72}   & %\multicolumn{1}{c|}{\textbf{0.73}}   & 0.47   & \textbf{0.58}   & %\textbf{0.62}   & \textbf{0.64}   \\
%GVM+learnt depth & -      & -      & -      & \multicolumn{1}{c|}{-}      & %0.45   & 0.56   & 0.60   & 0.62  
%\end{tabular}
%\caption{ \textbf{3D reconstructions  using randomly selected camera views.} %We show Intersection over Union (IoU) between the prediction and %groundtruth 3D voxel on ShapeNet. Notice how results improve with more %views. Learned depth is slightly worse than used groundtruth depth from a %depth sensor.}
%\label{tab:IoU_single_multi}
%\end{table}

\begin{table}[t!]
\centering
\begin{tabular}{c|cccccccc}
                  & \multicolumn{4}{c}{single object}                      & \multicolumn{4}{c}{multi-objects} \\ \cline{2-9} 
                  & view-1 & view-2 & view-3 & \multicolumn{1}{c|}{view-4} & view-1 & view-2 & view-3 & view-4 \\ \hline
 1D-LSTM           & 0.57   & 0.59   & 0.60   & \multicolumn{1}{c|}{0.60}   & 0.11   & 0.15   & 0.17   & 0.20   \\
LSM               & 0.63   & 0.66   & 0.68   & \multicolumn{1}{c|}{0.69}   & 0.43   & 0.47   & 0.51   & 0.53   \\
LSM+gt depth      & \textbf{0.65}   & 0.68   & 0.69   & \multicolumn{1}{c|}{0.70}   & \textbf{0.48}   & 0.51   & 0.54   & 0.56   \\
ours+gt depth     & 0.55   & \textbf{0.69}   & \textbf{0.72}   & \multicolumn{1}{c|}{\textbf{0.73}}   & 0.47   & \textbf{0.58}   & \textbf{0.62}   & \textbf{0.64}   \\
ours+learnt depth & -      & -      & -      & \multicolumn{1}{c|}{-}      & 0.45   & 0.56   & 0.60   & 0.62  
\end{tabular}
\caption{ \textbf{3D voxel occupancy prediction  using randomly selected camera views.} We show Intersection over Union (IoU) between the prediction and groundtruth 3D voxel grids. The performance of our model improves with more views. Using estimated depth as input does slightly worse than using  groundtruth depth.}
\label{tab:IoU_single_multi}
\end{table}
%For the single object case, we report mean IoU on three categories: chair, car, airplane.}

\begin{table}[t!]
\centering
\begin{tabular}{c|cccc|}
        & view-1 & view-2 & view-3 & view-4 \\ \hline
1D-LSTM & 0.12   & 0.16   & 0.16   & 0.18   \\
ours     & 0.24   & 0.28   & 0.31   & 0.32  
\end{tabular}
\caption{ \textbf{3D voxel occupancy prediction  using randomly selected camera views.} We show Intersection over Union (IoU) between the predicted  and groundtruth 3D voxel occupancies on SUNCG scenes.}
\label{tab:IoU_single_suncg}
\end{table}

\paragraph{Active view selection}
%To achieve better performance on 3D reconstruction, we apply an active module which selects the view that best aid on the final performance of 3D reconstruction. 
We evaluate the performance of our active view selection policy on 3D reconstruction of single and multiple objects. At each frame, our active observer learns to select an \textit{adjacent} ---as opposed to random  \cite{DBLP:journals/corr/abs-1709-00507}--- view to jump to,  in an attempt to mimic realistic deployment conditions on a robotic agent. 
We compare our learned  view selection policy with two baselines:
\begin{enumerate}
    \item \textit{random}, which randomly selects neighboring views to visit, and
    \item \textit{oneway}, which moves the camera along the same direction at each timestep so that the agent maximizes the horizontal or vertical baseline. 
    \item  \textit{1-step greedy},  similar to the one used in~\cite{3dshapenets}, which always selects the next view by maximizing the immediate increase in IoU for a single  step as opposed to a finite horizon. 
    \item \textit{oracle}, which selects the best among all possible view trajectories through exhaustive search. Since it is too expensive to try out all possible four-view-long trajectories, we sample 100 four-view-long trajectories and take the best as the oracle trajectory. This serves as an upperbound for our view selection policy.  
\end{enumerate}
We show quantitative results in Figure~\ref{fig:active_improve_all} and qualitative ones in Figure~\ref{fig:vis_1}.  The learned view selection outperforms the baselines for both single and multiple objects present. It better reconstructs detailed object parts, like the arm of a chair or the inside part of a mug. 
Compared to the \textit{oneway} policy, the \textit{active} policy select  views that ``undo" occlusions and recover most of the object. 

%To evaluate the effectiveness of our learned policy, we also compared our active policy with two other baselines: i) ii) Oracle view selection which is the best among all possible trajectories. 


We trained our policy using three random seeds  and report the mean and variance. 

%To be noted, oracle view selection serves as the upper bound for our learned policy. 
Percent increase in IoU between predicted and groundtruth voxel occupanices over single-view predictions are reported in Table~\ref{tab:IoU_single_increase}. We can see that our learned policy is worse than 1-step greedy policy in the first view, but outperforms it as more views become available. This is not surprising,  as our learned policy was trained to select views that  maximize the cumulative future rewards over a time horizon of four views. Qualitative results of the view selection policy are included in the Appendix. 
%For visualization of more camera trajectories generated by our view selector, please see the supplementary material. 

\begin{table}[b!]
\centering
\begin{tabular}{c|cccc}
\multirow{2}{*}{} & view-1 & view-2       & view-3       & view-4       \\ \cline{2-5} 
                  & \multicolumn{4}{c}{single object}                   \\ \hline
1-step greedy     & 0\%    & 29.1\%       & 32.7\%       & 33.3\%       \\
Active            & 0\%    & 27.7\%$\pm$3.23\% & 27.7\%$\pm$3.23\% & 36.6\%$\pm$1.17\% \\
Oracle & 0\%    & 32.7\%       & 38.1\%       & 38.1\%       \\ \hline
                  & \multicolumn{4}{c}{multi-objects}                   \\ \hline
1-step greedy     & 0\%    & 36.2\%       & 40.4\%       & 40.4\%       \\
Active            & 0\%    & 31.3\%$\pm$2.26\% & 39.0\%$\pm$1.99\% & 41.8\%$\pm$2.36\% \\
Oracle & 0\%    & 29.8\%       & 42.6\%       & 44.7\%      
\end{tabular}
\caption{ Percent increase in Intersection over Union (IoU) between 3D reconstructions and groundtruth over the single-view reconstruction. The first view is the same for all policies, so the IoU for the first view is the same.}
\label{tab:IoU_single_increase}
\end{table}

% and at the same time tries to move the camera as far as possible. 
%In Figure~\ref{fig:vis_1}, we show 3D 
%Reconstruction results obtained under our learned policy have higher quality on detailed parts like the arm of a chair or the inside of a mug. Learned view selection outperforms the baselines for both single and multiple objects present, as shown in Figure~\ref{fig:active_improve_all}. 

\input{imagegrid.tex}

\paragraph{Multi-view, multi-object  segmentation,  classification and 3D reconstruction}
No previous work has reported results on the task of object detection, segmentation and 3D reconstruction \textbf{under the presence of multiple objects occluding each other.} An important contribution of this paper is to address joint object instance segmentation, object category prediction and 3D reconstruction while accumulating information across multiple views in order to reveal occluded objects. We choose objects from four different categories, helmet, mug, bowl, and camera, that are similar in size. We place two objects in each scene between 0.25 and 0.35 units from the origin. The line passing through the centroid of both objects also goes through the origin. The scene is randomly rotated between $-90^{\circ}$ and $90^{\circ}$ degrees. 
\todo{how many scenes were used in train and how many in test?}
Although we only generated 332 scenes, our network is able to perform and generalize well.

We retrain the model of \cite{LSM} using our proposed state estimation loss functions and with absolute groundtruth camera poses as a comparison.
We report multi-object 3D reconstruction (voxel occupancy prediction) in Table~\ref{tab:IoU_single_multi} and classification and segmentation in Table~\ref{tab:seg3Dtable}. For 3D reconstruction, learned  depth always results in lower reconstruction IoU in each view. The proposed architecture outperforms LSM, and depth input always helps, even if it is estimated by a network as opposed to groundtruth. This result is encouraging given the improvement of depth sensors currently available that the proposed geometry-aware architecture can maximally take advantage of.  %and generalizes better. %But still, we outperform LSM w/o depth input.
For object segmentation, we compute the 3D IoU using the optimal matching between the segmented 3D voxel groups recovered from $k$-means and the groundtruth 3D object voxel grids. We report the average IoU across all objects in a scene. We also report classification accuracy. Table~\ref{tab:seg3Dtable} shows the quantitative results, and Figure ~\ref{fig:vis_seg} and ~\ref{fig:segmentation2D} shows visualizations of the instance segmentation and classification.


%The relative position between objects appeared in the scene and centroid of the scene are randomly sampled from $(\rho, \theta) \sim (U(0.25,0.35), U(-90^{\circ}, 90^{\circ}))$ where $U(x,y)$ is uniform distribution with lower bound of $x$ and higher bound of $y$. To ensure the two objects will occlude each other, $\theta_2 = \theta_1 + 18-^{\circ}$. 
%We compare the proposed model and LSM by training with the reconstruction loss using both ground truth and learned depth as input. In addition, we train our model with a segmentation embedding loss and a classification loss. 


\begin{comment}


\begin{figure}[t!]
    \centering
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/gt_depth.png}
    \end{minipage}
    \begin{minipage}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/depthnet.png}
    \end{minipage}
    
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/chair_new.png}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}
       \centering
        \includegraphics[width=\textwidth]{figures/curves/car_new.png}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/airplane_new.png}
    \end{minipage}
    \caption{Improvement in IoU among views using different policy. The upper left figure shows our method using groundtruth depth and mask and the upper right figure shows our method using learnt depth and mask on multi-objects. The three figures in bottom shows the results on three different categories: chair, car, airplane. Both of those results are yield by our method using groundtruth depth and mask.}
    \label{fig:active_improve_all}
\end{figure}
\end{comment}


\begin{figure}[t!]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/gt_depth.png}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/depthnet.png}
    \end{minipage}
      \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/chair_new.png}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}
       \centering
        \includegraphics[width=\textwidth]{figures/curves/car_new.png}
    \end{minipage}
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/curves/airplane_new.png}
    \end{minipage}
    \caption{\textbf{Improvement in 3D reconstruction IoU across views using different view selection policies.} \textit{Top row:} Multi-object scenes. \textit{Bottom row:} Single object scenes. Learned active policy outperforms alternatives by choosing trajectories that ``undo" occlusions.}
    \label{fig:active_improve_all}
\end{figure}

%\paragraph{Segmentation and Classification}

\begin{figure*}[t!]
    \centering
    \setlength{\tabcolsep}{0.05em}
    \begin{tabular}{ccccccccccccc}
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont Input} &
        \image{figures/seg/seg_28/rgb0.png} &
        \image{figures/seg/seg_28/rgb1.png} &
        \image{figures/seg/seg_28/rgb2.png} &
        \image{figures/seg/seg_28/rgb3.png} &
        \image{figures/seg/seg_42/rgb0.png} &
        \image{figures/seg/seg_42/rgb1.png} &
        \image{figures/seg/seg_42/rgb2.png} &
        \image{figures/seg/seg_42/rgb3.png} & 
        \image{figures/seg/seg_43/rgb0.png} &
        \image{figures/seg/seg_43/rgb1.png} &
        \image{figures/seg/seg_43/rgb2.png} &
        \image{figures/seg/seg_43/rgb3.png} \\
        
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont Ours} &
        \image{figures/seg/seg_28/img_v0.jpeg} &
        \image{figures/seg/seg_28/img_v1.jpeg} &
        \image{figures/seg/seg_28/img_v2.jpeg} &
        \image{figures/seg/seg_28/img_v3.jpeg} &
        \image{figures/seg/seg_42/img_v0.jpeg} &
        \image{figures/seg/seg_42/img_v1.jpeg} &
        \image{figures/seg/seg_42/img_v2.jpeg} &
        \image{figures/seg/seg_42/img_v3.jpeg} & 
        \image{figures/seg/seg_43/img_v0.jpeg} &
        \image{figures/seg/seg_43/img_v1.jpeg} &
        \image{figures/seg/seg_43/img_v2.jpeg} &
        \image{figures/seg/seg_43/img_v3.jpeg} \\
        
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont gt} &
        \image{figures/seg/seg_28/gt.jpeg} &
        \image{figures/seg/seg_28/gt.jpeg} &
        \image{figures/seg/seg_28/gt.jpeg} &
        \image{figures/seg/seg_28/gt.jpeg} &
        \image{figures/seg/seg_42/gt.jpeg} &
        \image{figures/seg/seg_42/gt.jpeg} &
        \image{figures/seg/seg_42/gt.jpeg} &
        \image{figures/seg/seg_42/gt.jpeg} & 
        \image{figures/seg/seg_43/gt.jpeg} &
        \image{figures/seg/seg_43/gt.jpeg} &
        \image{figures/seg/seg_43/gt.jpeg} &
        \image{figures/seg/seg_43/gt.jpeg} \\
    \end{tabular}
    \caption{Visualization results of 3D segmentation on multi-object scenes.}
    \label{fig:vis_seg}
\end{figure*}



\begin{table}[htbp!]
\centering
\begin{tabular}{c|cccc}
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{view-1} & \multicolumn{1}{l}{view-2} & \multicolumn{1}{l}{view-3} & \multicolumn{1}{l}{view-4} \\ \hline
3D reconstruction IoU & 0.54 & 0.63 & 0.64 & 0.65 \\
3D segmentation IoU                  & 0.60   & 0.69   & 0.70   & 0.71   \\
Classification accuracy    & 0.56 & 0.83 & 0.83 & 0.83
\end{tabular}
\caption{ \textbf{3D object segmentation and classification using two objects per scene and four object categories.} As expected, both reconstruction and segmentation IoU increase with more views. The four object categories are roughly balanced and always guessing the most common category yields  32\% accuracy.}
\label{tab:seg3Dtable}
\end{table}

\begin{figure}[htbp!]
    \centering
    \begin{minipage}{0.98\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/segcls3d.png}
    \end{minipage}
    \caption{\textbf{Object segmentation under occlusions}. We are able to project the segmented 3D voxels and obtain amodal bounding boxes and segmentation masks, even in the presence of heavy occlusions. We show segmentations specifically from the most heavily occluded camera views.}
    \label{fig:segmentation2D}
\end{figure}

\paragraph{Sensitivity to egomotion estimation errors}
Our reconstruction method uses the relative camera pose between views in order to align the unprojected feature tensors. However, there may be camera pose estimation errors in a realistic environment. We test the robustness of our model to such errors by adding random noise to azimuth and elevation. We consider noise  distributed normally with $\mu = 0$ and $\sigma = 5\ \text{degrees}$ for both the azimuth and elevation. We test noise which is independent for each view, and also noise that accumulates across views, so that the error at view $i$ is the error at view $i-1$ plus the error at view $i$. This means that last  feature tensor is subjected to the greatest amount of alignment error. We test two variants of our method: one trained without noisy egomotion, and one trained with (independent) noisy egomotion. We show quantitative results in Table~\ref{tab:poseerror}. 

\begin{table}[htbp!]
\centering
\begin{tabular}{c|cc}
            \multicolumn{1}{l|}{}          &  \multicolumn{1}{l}{Trained without noise} & \multicolumn{1}{l}{Trained with noise} \\ \hline
groundtruth egomotion      & \textbf{0.64}   & 0.63     \\
Independent egomotion noise   & 0.56   & \textbf{0.59}    \\
Accumulating egomotion noise      & 0.56   & \textbf{0.58}    \\
\end{tabular}
\caption{\textbf{3D reconstruction under noisy egomotion}  for the chair category. We show IoU for the different test-time scenarios listed in the left column. The performance of our model degrades gracefully with noise in egomotion estimation. Moreover, when trained with such noise, it  become more resistant to such errors.}
\label{tab:poseerror}
\end{table}

%As we show in Table~\ref{tab:poseerror},  
%the performance of our model degrades gracefully with noise, and that it is possible to train the network to become more resistant to such errors. \todo{ricson: this last bit what does it mean???}

==> imagegrid2.tex <==
\begin{figure*}[t!]
    \centering
    \setlength{\tabcolsep}{0.05em}
    \begin{tabular}{ccccccccccccc}
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont Input} &
        \image{figures/visual/air_1/rgb/rgb0_oneway.png} &
        \image{figures/visual/air_1/rgb/rgb1_oneway.png} &
        \image{figures/visual/air_1/rgb/rgb2_oneway.png} &
        \image{figures/visual/air_1/rgb/rgb3_oneway.png} &
        \image{figures/visual/chair_1/rgb/rgb0_oneway.png} &
        \image{figures/visual/chair_1/rgb/rgb1_oneway.png} &
        \image{figures/visual/chair_1/rgb/rgb2_oneway.png} &
        \image{figures/visual/chair_1/rgb/rgb3_oneway.png} & \image{figures/visual/dm_1/rgb/rgb0_oneway.png} &
        \image{figures/visual/dm_1/rgb/rgb1_oneway.png} &
        \image{figures/visual/dm_1/rgb/rgb2_oneway.png} &
        \image{figures/visual/dm_1/rgb/rgb3_oneway.png} \\
        
        \rotatebox[origin=c]{90}{\parbox{1cm}{\fontsize{8}{9.6}\selectfont \centering 2D \\ \centering LSTM}} &
        \image{figures/visual/air_1/2d/img_v0.jpeg} &
        \image{figures/visual/air_1/2d/img_v1.jpeg} &
        \image{figures/visual/air_1/2d/img_v2.jpeg} &
        \image{figures/visual/air_1/2d/img_v3.jpeg} & \image{figures/visual/chair_1/2d/img_v0.jpeg} &
        \image{figures/visual/chair_1/2d/img_v1.jpeg} &
        \image{figures/visual/chair_1/2d/img_v2.jpeg} &
        \image{figures/visual/chair_1/2d/img_v3.jpeg} &
        \image{figures/visual/dm_1/2d/img_v0.jpeg} &
        \image{figures/visual/dm_1/2d/img_v1.jpeg} &
        \image{figures/visual/dm_1/2d/img_v2.jpeg} &
        \image{figures/visual/dm_1/2d/img_v3.jpeg} \\
        
      
        
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont GVM} &
        \image{figures/visual/air_1/oneway/img_v0.jpeg} &
        \image{figures/visual/air_1/oneway/img_v1.jpeg} &
        \image{figures/visual/air_1/oneway/img_v2.jpeg} &
        \image{figures/visual/air_1/oneway/img_v3.jpeg} & \image{figures/visual/chair_1/oneway/img_v0.jpeg} &
        \image{figures/visual/chair_1/oneway/img_v1.jpeg} &
        \image{figures/visual/chair_1/oneway/img_v2.jpeg} &
        \image{figures/visual/chair_1/oneway/img_v3.jpeg} &
        \image{figures/visual/dm_1/oneway/img_v0.jpeg} &
        \image{figures/visual/dm_1/oneway/img_v1.jpeg} &
        \image{figures/visual/dm_1/oneway/img_v2.jpeg} &
        \image{figures/visual/dm_1/oneway/img_v3.jpeg} \\
        
        \rotatebox[origin=c]{90}{\parbox{1cm}{\fontsize{8}{9.6}\selectfont Input \\ active}} &
        \image{figures/visual/air_1/rgb/rgb0_active.png} &
        \image{figures/visual/air_1/rgb/rgb1_active.png} &
        \image{figures/visual/air_1/rgb/rgb2_active.png} &
        \image{figures/visual/air_1/rgb/rgb3_active.png} &
        \image{figures/visual/chair_1/rgb/rgb0_active.png} &
        \image{figures/visual/chair_1/rgb/rgb1_active.png} &
        \image{figures/visual/chair_1/rgb/rgb2_active.png} &
        \image{figures/visual/chair_1/rgb/rgb3_active.png} &
        \image{figures/visual/dm_1/rgb/rgb0_active.png} &
        \image{figures/visual/dm_1/rgb/rgb1_active.png} &
        \image{figures/visual/dm_1/rgb/rgb2_active.png} &
        \image{figures/visual/dm_1/rgb/rgb3_active.png} \\
        
        \rotatebox[origin=c]{90}{\parbox{1cm}{\fontsize{8}{9.6}\selectfont GVM \\ active}} &
        \image{figures/visual/air_1/active/img_v0.jpeg} &
        \image{figures/visual/air_1/active/img_v1.jpeg} &
        \image{figures/visual/air_1/active/img_v2.jpeg} &
        \image{figures/visual/air_1/active/img_v3.jpeg} & \image{figures/visual/chair_1/active/img_v0.jpeg} &
        \image{figures/visual/chair_1/active/img_v1.jpeg} &
        \image{figures/visual/chair_1/active/img_v2.jpeg} &
        \image{figures/visual/chair_1/active/img_v3.jpeg} &
        \image{figures/visual/dm_1/active/img_v0.jpeg} &
        \image{figures/visual/dm_1/active/img_v1.jpeg} &
        \image{figures/visual/dm_1/active/img_v2.jpeg} &
        \image{figures/visual/dm_1/active/img_v3.jpeg} \\
        
        \rotatebox[origin=c]{90}{\fontsize{8}{9.6}\selectfont gt} &
        \image{figures/visual/air_1/gt.jpeg} &
        \image{figures/visual/air_1/gt.jpeg} &
        \image{figures/visual/air_1/gt.jpeg} &
        \image{figures/visual/air_1/gt.jpeg} & 
        \image{figures/visual/chair_1/gt.jpeg} &
        \image{figures/visual/chair_1/gt.jpeg} &
        \image{figures/visual/chair_1/gt.jpeg} &
        \image{figures/visual/chair_1/gt.jpeg} &
        \image{figures/visual/dm_1/gt.jpeg} &
        \image{figures/visual/dm_1/gt.jpeg} &
        \image{figures/visual/dm_1/gt.jpeg} &
        \image{figures/visual/dm_1/gt.jpeg} \\
    \end{tabular}
    \caption{\textbf{3D reconstruction results} on single and multiple objects using different methods. Note the ability of our model to model the thin armrest of the chair without blending it into the body.}
    \label{fig:vis_1}
\end{figure*}

==> intro4.tex <==

%\textit{``When we will figure out how to use 3D representations, no one would ever use 2D again, same as when color TV was invented, no one watched black and white."} Yaser Sheikh

\section{Introduction}

Current state-of-the-art object detectors \cite{DBLP:journals/corr/RenHG015}, despite their formidable performance increase in recent years, carry the biases and idiosyncrasies of the data they were trained on \cite{DBLP:journals/corr/abs-1711-03213}: static images from Imagenet and COCO datasets. Thus, detectors do well on viewpoints that human photographers tend to prefer, but may fail on images (non skillfully) captured by robotic agents, that %are not trained to focus attention on visual input in  intelligent ways (see Figure \ref{fig:motivation}), but rather 
often feature severe cross-object occlusions and viewpoints which are unusual for humans. %, or with important visual content outside their field of view. % pose persistent difficulties to static object detectors.
Robotic agents on the other hand do not abide by the constraints of \textit{passive} vision: they can actively \textit{choose where to look} in order to recover from occlusions and difficult viewpoints, a problem well-known under the name active vision \cite{activealoimonos}. %, and facilitate   object segmentation, classification and 3D reconstruction,  
%of their environments, and in this way 
%and . 
%In fact, the field of active vision \cite{activealoimonos} %in its early development 
%advocates precisely this: 
%Actively selecting camera parameters to minimize sensing uncertainty is known as active vision \cite{activealoimonos}. 
It has been argued that without such active view selection, 
%Recent research claims that unless  visual observers can actively collect new information, we cannot provide 
no formal performance guarantees can be provided for visual recognition algorithms \cite{soat}. 



We propose \textbf{geometry-aware 3D visual memory architectures and loss functions for active object detection, segmentation and 3D reconstruction  in cluttered scenes},  following the old active vision premise. 
Paradoxically, recent methods trained to actively accumulate information across visual glimpses/ camera views have been applied either for object detection/recognition in \textit{passive static} images \cite{mathe,fer,aolw}, or for reconstruction of  \textit{isolated}  objects in actively collected  views  \cite{DBLP:journals/corr/abs-1709-00507}.   In passive images, we cannot undo occlusions and recover necessary missing information, as advocated by the principle of the moving observer \cite{soat}. In actively collected images, 
%of  with recurrent neural networks \cite{} and address object detection in 2D by active glimpse selection to fight feature contamination from context, but also in  3D for 
%3d reconstruction of  \textit{isolated}  objects \cite{DBLP:journals/corr/abs-1709-00507}.   
delineating the object of interest from a cluttered scene   %We advocate that such framing of the problem is in fact against the active vision premise: focusing on a particular object is unrealistic under clutter, in fact, object clutter 
%is precisely what active vision is supposed to address, 
is often a  harder problem than reconstructing or classifying once  isolated from clutter  \cite{3dshapenets,LSM}. 
To the best of our knowledge, this work is the first to attempt the full state estimation problem  in cluttered  scenes with cross-object occlusions. Our main contribution is a geometrically-consistent 3D memory architecture that accumulates information from actively selected camera views into a 3D feature map of the scene. \textbf{Object segmentation, classification and 3D reconstruction is directly solved for from the output of the 3D feature memory, as opposed to in 2D images}, where objects occlude one another. In this way, object delineation improves with more views. This is drastically different from the paradigm of tracking by detection where we need to commit to object detections in every view and correspond them in time,  and often suffers from early erroneous decisions \cite{WongRSSWS13}. Solving for object detection from 3D  information directly allows to accumulate multiple views necessary to detect the objects reliably. %The segmented 3D voxel grid is projected to 2D according to predicted scene depth and generates amodal detection boxes for the objects in the heavily occluded input 2D views.
Camera projection of 3D object segments generates amodal category labelled boxes and segmentations in the (potentially heavily) occluded input 2D views.
%, which is a paradox of the active vision paradigm in 3D scenes \cite{edshapenets}. % It is a harder problem than classifying an isolated uncluttered object. % itself.%Thus framing the problem in this way is unrealistic. 
%We have empirically validated that 
%We have empirically found that  2D  recurrent neural architectures, often used by recent active vision approaches \cite{},   do not effectively generalize in clutter due to combinatorial explosion of  occlusion configurations, which may explain    %to the minimum clutter: 2D convolutional LSTM or GRU units simply cannot deal with occlusions and effectively generalize across occlusion configuration. 
%Such performance limitations potentially limits 
%limiting the problem scope to isolated objects. % for active view selection in previous works. %information accumulation across camera viewpoints is currently hindered by the 2D nature of recurrent networks. 



 
%We propose \textbf{geometry-aware visual memory architectures and cost functions for active state estimation, namely, object detection, segmentation and 3D reconstruction  in cluttered   scenes}. 
In a nutshell, our method works as follows. At each time step, the proposed active observer selects a nearby camera view. 
It then  ``unprojects"  RGB, (learned) depth and object foreground  channels into a 3D feature tensor, which is rotated to match the pose of the first camera view, using the relative egomotion. The warped feature tensor updates a 3D memory latent state map of a convolutional Gated Recurrent Unit (GRU) layer. Geometric memory consistency ensures that \textit{2D  projections of the same 3D physical point are placed nearby in the 3D feature memory tensor},  a key for generalization. %, in contrast to 2D geometry-unaware alternatives \cite{}.
%Egomotion-transformed 3D features are aggregated using 3D convolutional GRUs. 
GRU convolutional filters can then ``see" information regarding the same 3D concept in their viscinity. They transform it  into higher level features optimized for object instance segmentation, classification and voxel occupancy prediction, directly in 3D. 
%in the input and novel camera views. 
Our geometry-aware visual memory   is trained  end-to-end in a  differentiable manner, and our active view selection is trained with reinforcement based on state estimation accuracy in each view. 
%. The top layer 3D feature map is mapped to segmentation embeddings, label classification and voxel occupancy outputs. %which are translated inot 
%Our active observer chooses the next nearby view to visit to maximize performance in detecting, segmenting and 3D reconstructing the objects in the visual scene. 

%In each view, our agent predicts a depth map and unprojects image and predicted depth information in a 3D tensor grid, after aligning it to the original viewpoint based on cumulative camera motion estimate. 
%Features are computed in this unprojected feature grid and are accumulated with feature thus far using a 3D convolutional GRU. Our egomotion aware unprojection, ensures that features from 2D projections of the same 3D physical points lie nearby on the 4d tensor, which is the key to generalization in comparison to 2D egomotion unaraware alternatives.  the cumulative features result in multiple heads where feature embedding are optimized for 3D grouping and reconstruction of the scene. the segmented 3D grid, trivial is projected to amodal detection boxes in the input and novel views. Our reconstruction architecture is train in an end to end differentiable manner, while our active observer uses an actor critic architecture and is optimized for state estimation performance in each view. 
%Depth reprojection losses allow test time unsupervised adaptation. 

%\todo{shall we mention camera motion? woultn it be cool if we could be supervised only by 2D information, depth and segmentation? (depth we have)}



%\todo{add here comparison to closest works and mention d=non comitment}

%\todo{mention this in the intro}, as opposed to  absolute poses of \cite{LSM}. 



%\todo{write more about marrying slam+learning}
We empirically show the proposed 3D recurrent memory architecture  outperforms by a large margin 2D recurrent memory alternatives, convolutional or not, which  do not effectively generalize in cluttered scenes due to the combinatorial explosion of occlusion configurations. %, which may explain    %to the minimum clutter: 2D convolutional LSTM or GRU units simply cannot deal with occlusions and effectively generalize across occlusion configuration. 
 Our view selection policy outperforms naive or random view selection alternatives. The proposed method marries pure geometric localization and 3D pointcloud mapping \cite{schoeps14ismar}  with feature mapping from experience, while being robust to mistakes of depth and egomotion estimation. 
%It better fits visual recognition for active robotic observers, as opposed to passive observer of internet imagery.
%is a step towards vision for robotics as opposed to vidion for internet images. 
In summary our contributions are:

\begin{itemize}
    \item Introducing the problem of active state estimation, namely, selecting camera views for jointly optimizing object instance segmentation, classification and 3D reconstruction, a problem very relevant for robotic computer vision.
    
    \item Proposing a geometry-aware visual memory architecture that accumulates feature  information directly in 3D. The proposed memory model works for both passive as well as actively collected video sequences.
    %which does not need to commit early to object detection/segmentation as its 2D alternatives, and can be used both with active and passive video sequences
    
   % \item combining learning based view information woth depth reprojection losses for test time adaptation
    
    \item Conducting extensive experiments and ablations  against alternative memory architectures and alternative view selection policies, as well as for quantifying sensitivity of the proposed memory to accuracy of recovered geometric information regarding depth and egomotion. %, 3D RGB non active architectures 
\end{itemize}

Our code and datasets will be made publicly available upon acceptance.

%reinforcement learning 


%based on relative camera viewpoint. Feature are computed using 3D convolutions and are accumulated through a 3D convolutional GRU memory. The cumulative c

%and  and  a recurrent neural network architecture for active visual recognition that accumulates information directly in  a 3Dimensional feature volume 
%4D feature grid, where each  

 
%and are victims of occlusions: where they do not attempt to predict the full extent of the object. 

==> model_old.tex <==
\section{Active geometric-semantic visual recognition} \label{sec:model}
%\todo{ricson,ziyan to write}

We consider an active visual observer, e.g., a robotic agent,  equipped with a perspective camera model. 
The proposed active visual recognition model is illustrated in Figure \ref{fig:arch}. It is comprised of a differentiable short-term geometry-aware visual memory and an camera viewpoint selection policy. We detail each below.

\subsection{Short-term geometry-aware visual memory}
Our memory model is a recurrent neural network whose latent memory state is a 3D feature map of the visual scene. The memory map is updated with each new camera view in a geometrically consistent way, so that information from 2D pixel projections that correspond to the same 3D point  end up close by, allowing for convolutions with a necessarily limited receptive field to effectively process the multiview input. Given an RGB frame, we first predict a depth map and a foreground mask. Next, 2D depth, segmentation and RGB maps are ``lifted" into 3D using an unprojection operation, rotated to compensate for the egomotion, and then aggregated using a 3D convolutional Gated Recurrent Unit layer \cite{DBLP:journals/corr/ChoMGBSB14}. We will assume ground-truth egomotion information throughout the paper, similar to previous methods, since an active observer does have access to its approximate egomotion. We quantify how robust our memory architecture is to inaccurate egomotion in Section \ref{sec:experiments}. 

\begin{figure}[t!]
    \centering
    %\includegraphics[width=\textwidth]{figures/combine3.png}
    \includegraphics[width=\textwidth]{figures/figure4.png}
    % \caption{\textbf{Active geometric-semantic visual recognition} 
    % (a) Our active agent sequentially accumulates visual information in a 3D geometrically-consistent feature map of the visual scene. 
    % At each frame, the agent selects a nearby camera view, conditioned on the 3D feature map of the scene thus far, and the current RGB image. It  predicts a corresponding 2D depth map and foreground object mask. RGB, depth and segmentation maps are unprojected in corresponding 3D feature tensors,  mapped using the relative egomotion to the coordinate frame of the cumulative 3D feature map built thus far, and update a 3D convolutional GRU memory.   The output of the 3D GRU memory is then  mapped via a 3D encoder-decoder network to segmentation embeddings, object category probabilities, and occupancy for every voxel in the 3D grid. (b) \textbf{Unprojection.} RGB and depth values are unprojected  to 3D following camera rays (undoing camera projection).   
    % }
    \caption{\textbf{Active geometric-semantic visual recognition} 
    Our active agent sequentially accumulates visual information in a 3D geometrically-consistent feature map of the visual scene. 
    At each frame, the agent selects a nearby camera view, conditioned on the 3D feature map of the scene thus far, and the current RGB image. It  predicts a corresponding 2D depth map and foreground object mask. RGB, depth and segmentation maps are unprojected in corresponding 3D feature tensors, mapped using the relative egomotion to the coordinate frame of the cumulative 3D feature map built thus far, and update a 3D convolutional GRU memory. The output of the 3D GRU memory is then  mapped via a 3D encoder-decoder network to segmentation embeddings, object category probabilities, and occupancy for every voxel in the 3D grid.
    }
    \label{fig:arch}
\end{figure}

\paragraph{Unprojection}

%In the unprojection step, 
For each camera view, our model is given the RGB image and predicts the corresponding 2D depth and object foreground map with a 2D convolutional encoder-decoder model with skip-connections. It then unprojects those to fill in an initial 3D feature tensor as follows:

For each feature voxel $V_{i,j,k}$ in the 3D tensor we compute the pixel location $(x,y)$ which it projects onto, from the current camera view. Then, $V_{i,j,k}$ is filled with the bilinearly interpolated RGB, depth and mask at $(x,y)$. All voxels lying along the same ray shot from the camera will be filled with nearly the same RGB, depth and mask, although in practice, since the centroids of two voxels are rarely on the exact same camera ray, the features will differ slightly. %We use the perspective camera model.
%An additional step of the unprojection operation that previous works (cite lsm here) do not use is to explicitly 

We further compute (i) a grid of depth values, so that $V_{i,j,k} = k$ and (ii) a binary voxel occupancy grid containing the thin shell of voxels directly visible from the current camera view. We compute this by filling all voxels whose unprojected depth value equals the grid depth value. Thus, our unprojection operation results in an initial feature tensor $\mathcal{M}^{64 \times 64 \times 64 \times 7}$: 3 channels for RGB, 2 channels for depth and mask, 1 channel for the surface occupancy, and 1 channel for the grid of depth values. We visualize the unprojection operation for one slice of the 3D tensor in Figure \ref{fig:arch} (b). We will call the proposed operation \textit{early} unprojection to distinguish from the one used in \cite{LSM}, which unprojects 2D convolutional features instead of RGB, mask and depth input. We compare against \cite{LSM} in Section \ref{sec:experiments}. %An illustration of unprojection is shown  Figure~\ref{fig:arch} (b). 


\paragraph{Recurrent memory update}
In order for 2D projections of the same physical point to end up close by in our 3D memory tensor, in each view, we rotate unprojected feature tensors to the orientation of the first camera view. This requires only relative camera pose (egomotion). 
At each time step, once the feature tensor has been properly oriented, we apply a 3D convolutional layer, and then update a 3D convolutional GRU memory layer. The operation of how GRU memory layer update can be expressed as:
\begin{align}
    h_{t+1} &= u_t\circ h_t + (1-u_t)\circ \tanh(\text{conv3d}([x_t,r_t\circ h_t], W_h)) \\
    u_t, r_t &=\sigma(\text{conv3d}([x_t,h_t],[W_u, W_r]))
\end{align}
where $u_t$ and $r_t$ are the GRU update gate and reset gate respectively.
We experimented max pooling and average pooling strategies, but found that GRU accumulation worked best. 

\paragraph{Object reconstruction, instance segmentation and classification}

The output of the 3D GRU memory is fed into a 3D convolutional encoder/decoder network with skip-connections to produce (i) a 3D sigmoid output which predicts voxel occupancy, (ii) a 3D segmentation embedding tensor, and (iii) a multiclass softmax output at every voxel for classification. The embeddings and classification outputs are at half the resolution of the occupancy grid.

We train for 3D reconstruction using a standard binary cross-entropy loss. We train the instance segmentations using metric learning and a standard contrastive loss \cite{Hadsell06dimensionalityreduction}, that pulls segmentation embeddings of voxels of the same object instance close, and pushes segmentation embeddings of different object instances (and the empty space) apart. For metric-learning, during training, we sample the same number of voxel examples from each object instance to keep the loss balanced, not proportional to the volume of each. 

We then convert the segmentation embeddings into a hard segmentation decision. First we collect the embeddings in voxels whose predicted occupancy is greater than 0.5. Then we run the K-Means algorithm on these features, with $k$ set to the number of objects in the scene, in order to bin each voxel into one of $k$ sets. 

When the number of objects is unknown, we oversegment the scene using a large $k$ as shown in Figure \ref{fig:oversegmentation}, and then merge iteratively merge clusters where the ratio of the number of border voxels to the volume of the larger of the two clusters, $R$, is maximized. We stop merging when $R < 1.5$. 

\begin{figure}[b]
    \centering
    \includegraphics[width=\textwidth]{figures/oversegmentation.png}
    \caption{The left image in each pair shows the oversegmented scene using $k = 8$. We merge the clusters in order to obtain the final segmentation on the right}
    \label{fig:oversegmentation}
\end{figure}

For each group resulting from the K-means algorithm, we compute the average of the logits predicted for the voxels in that group. We train with cross-entropy loss between the average logit and the ground truth class label of the shape in the scene which has the highest IoU with that group. 

\subsection{Learning to select the best adjacent view}


%We treat the next view selection  as a partially observable markov decision process, thus 

We train a view selection policy network that outputs, at each timestep, a distribution over eight adjacent camera views in the neighborhood of the current one. 
The policy network is a two branch convolutional neural network. The input to the 3D branch is the output of the GRU memory layer, and the input to the 2D branch is the current RGB image. They are both mapped, using 3D and 2D convolutions respectively, to a final 1D vector after flattening and concatenating. A fully connected layer with softmax activation produces the final  categorical distribution over 8 possible directions. The exact architecture of the view selection policy is included in the supplementary material. 
%The network takes as input the output of the 3D convGRU memory and RGB iamge of time step $t$ and produces a categorical distribution over 8 possible directions. The policy network has two branches of input, one for current view RGB image with 2D conv layers, another for 3D aggregated features with 3D conv layers. Then the extracted features of the two branches are flattened and concatenated along the last axis. A fully connected layer with softmax activation outputs the final distribution $\pi(a_t|s_t, \theta)$ from the features extracted from $\mathcal{I}(t)$ and $V(t)$ as input.


  We train our policy network with REINFORCE \cite{sutton2000policy} with a baseline, a standard reinforcement learning algorithm. The policy $\pi(a_t|s_t, \theta)$ is iteratively updated by applying gradient ascent to maximize the expectation of total reward. The policy gradient reads:
\begin{equation}
    g(s) = E_t[\nabla_{\theta} \log(\pi_{\theta}(a_t|s_t, \theta))R_t],
    \label{nonumber}
\end{equation}
where $R_t$ is the reward of step $t$ and $\pi_{\theta}(a_t|s_t, \theta)$ is the trainable policy network. $E_t[\cdot]$ is the empirical expectation of the average over a finite number of sampled time steps. Though our observer solves for joint object segmentation, classification and 3D reconstruction, we found it adequate to indicate reconstruction-driven rewards  $R_t$, as the  \textit{increase} in Intesection over Union (IoU) of the discretized voxel occupancy from each view to the next.


%In our 3D reconstruction setting, we define the reward $R_t$ to be the increase in IoU of the voxel occupancy from one view to the next. 



==> pitch.tex <==
We are proposing a framework for visual recognition that takes into account information across multiple  views (camera viewpoints) of the navigating agent. Deep features are aggregated in 3D feature embedded maps, in a geometrically-consistent way, by taking into account the egomotion of the agent for transforming 2d deep feature maps, before aggregating them into the 3D memory. Then, object detection and classification will be carried out directly from the aggregated 3D feature map, as opposed to single 2d views, robust to occlusions. This is a drastically different paradigm for object recognition than per frame 2D object detection, used currently for object recognition in videos. Preliminary results show such geometrically-consistent multiview deep feature integration results in much higher performance than tracking by detection, which early commits to object bounding boxes, decisions that are hard to correct in an end-to-end differentiable way, as more video information is revealed. We further trained a view selection policy to result in view sequence most useful for object detection from the accumulated 3d feature map."

==> related_work.tex <==
\section{Related Works}

\paragraph{Active vision}
An active vision system is one that can manipulate the viewpoint of the camera(s) in order to explore the environment and get better information from it \cite{ap,aor}. Active visual recognition attracted attention as early as 1980's. The work of \cite{activealoimonos} suggested many problems such as shape from contour and structure from motion, while ambiguous for a passive observer, they can easily be solved for an active one \cite{1238372,blur}. 
%Researchers attempted to select zoom in/zoom out settings for object tracking\cite{1238372}, minimize motion blur \cite{blur}, enhancing depth perception of an object by focusing two cameras on the same object or moving the cameras \cite{activealoimonos}. 
Active control of the camera viewpoint also helps in focusing computational resources on the relevant elements of the scene \cite{doi:10.1167/11.5.5}. The importance of active data collection for sensorimotor coordination has been highlighted in the famous experiment of Held and Hein  in 1963 \cite{kitten}, involving two kittens engaged soon after birth to move and see in a carousel apparatus. The active kitten that could move freely was able to develop healthy visual perception, but the passively moved around kitten suffered significant deficits. %one was  the rolling cats: though two kitten observed the same series of visual scenes, the kitten that was selecting the scenes learnt while the kitten that was carried around passively obsering was not able to learn.
%\todo{can someone collect active vision references maybe fro our related paper? We need some very old citations, and how these old works are different than current reinforcement learning methiods}
%The birth of Computer Vision in fact started with approaches that were trying to decide where to look for obstacle avoidance as opposed to explain what they are looking at. Such methods were active vision as they were developed having in mind an active robotic agents. 
Despite its  importance, active vision was put aside potentially due to the slow development of autonomous robotics agents, necessary for the realization of its full potential. 
%Many researchers shifted attention to recognition from large static image collections \cite{} and use of big data neural networks. 
Recently, the active vision paradigm has been resurrected by approaches that perform selective attention \cite{where} and selective sequential image glimpse  processing in order to accelerate   object localization  and recognition    in 2D static images \cite{mathe,fer,aolw}.  Fewer methods have addressed    camera view selection for a moving observer \cite{dfd,tdvn,DQL}, e.g. for navigation \cite{kavu,gup} or for object 3d reconstruction, in synthetic environments  \cite{DBLP:journals/corr/abs-1709-00507}. 
%object recognition and localization methods in 2d images 
%have re
%image based reinforcement learning methods have resurrected the old idea \cite{} by learning to select camera in synthetic environments: using 3d synthetic object models, they attempt to choose the next best view to improve 3d object reconstruction. 
Many of the aforementioned approaches  use some type of recurrent network \cite{mathe,fer,aolw,DBLP:journals/corr/MnihHGK14,LSM} that  accumulates information across views or glimpses. 
%The latent state  is then mapped to a 3d voxel occupancy grid \cite{DBLP:journals/corr/abs-1709-00507} or object category label \cite{}. 
Since we cannot backpropagate through view or glimpse  selection, reinforcement learning methods have often been  used to train  view or glimpse selection policies.   

%3D ShapeNets \cite{song2016im2pano3d} introduces a non-RL based method for view selection: they use a generative model for 3D shapes, and then select the view which maximizes the information gain, as computed by sampling possible shapes from the generative model. However, we show that this greedy-approach is suboptimal. \todo{we need to fix this description}
%Our work proposes architectures for an active agent that performs full state estimation in a cluttered visual scene, a more realistic setup compared to recognition or reconstruction of isolated objects, for which active vision would have been necessary.  The proposed geometry-aware recurrent neural network outperforms by a margin geometry-unaware alternatives in the presence of multiple objects, even with small data supervision. 


%in a more natural setup, that of 
%full state estimation in a cluttered input scene, as opposed to isolated objects. The active observer attempts to dilleneate the objects, detect, segment, 3d reconstruct them, i.e.,  optimize for a full state estimation as opposed to single object 3d reconstruction. %Our depth-aware geometric accumulator can be optimized either with reprojected segmentation and depth or directly in 3d when information is available. 
%The proposed geometry-aware memory architecture better matches the visual domain and we , and allows active accumulation of information for undoing cross-object occlusions, the main source of information loss, that genrated an exponentation number of conifgurations in contast to self-occlusions.
%While works of \cite{DBLP:journals/corr/abs-1709-00507} permit their active observer to select any random camera view,  our active observer optimizes for the next best \textit{nearby} view, and thus presents a more realistic setup for a robotic agent that cannot spontaneously look all around a scene, but rather nearby.

\paragraph{Deep geometry} 
%Our differentiable rendering  architecture build upon recent works that = integrate deep learning into geometric inference. 
There has recently been great interest in integrating learning and geometry for single view 3D object reconstruction  \cite{DBLP:journals/corr/TulsianiZEM17, DBLP:journals/corr/abs-1711-03129}, depth and egomotion estimation from pairs of frames \cite{sfmnet,tinghuisfm}, depth estimation from stereo images \cite{DBLP:journals/corr/GodardAB16}, estimating 3D locations of human keypoints from 2D keypoint heatmaps \cite{3dinterpreter,DBLP:journals/corr/TungHSF17}. Many of those works use neural network architectures equipped with some form of differentiable camera projection, so that 3D desired estimates can be supervised directly using 2D quantities.  They do not accumulate information across multiple camera viewpoints. For example, works of \cite{DBLP:journals/corr/TulsianiZEM17, DBLP:journals/corr/abs-1711-03129,tinghuisfm} use a single image frame to predict 3D reconstruction of a single object, or a 2D depth map of the entire scene, though they use multiple views to obtain supervision in the form of depth re-projection error.  Works that use reprojection error as  self-supervision at test-time \cite{3dinterpreter,DBLP:journals/corr/TungHSF17,sfmnet,tinghuisfm,DBLP:journals/corr/TulsianiZEM17, DBLP:journals/corr/abs-1711-03129} cannot operate in an online, interactive mode  since backpropagating  error gradients takes time. We have not observed empirical gains from incorporating such self-supervised depth reprojection losses in our model.  
%Moreover, we show in Section \ref{sec:experiments} that our method that explicitly learns to accumulate  information across multiple views outperforms those methods that use multi-view supervision through reprojection.\todo{that last sentence needs to be revised later} 
The authors of \cite{pointnet} propose neural network architectures that operate  directly with  3D pointcloud input, as opposed to pixel grids. They do not accumulate information across multiple views. 

\todo{the follfowing description is super incomprehensible}
Im2Pano3D \cite{song2016im2pano3d} extrapolates a partial RGB view of a scene to a semantic map of the entire panorama. They also embed prior knowledge about camera geometry into their network by using what they call a "PN-Layer". Their work differs from ours in that they do not attempt to aggregate information across multiple views, and therefore do not need a memory.

%Works of \cite{deepmind,diffraycatsing} learn a mapping from 2d depth input to full 3d reconstruction and use differentiable projection to supervise themsevles from 2d quantities. 

%Similarly \cite{3dinterpeter} predicts 3d locations of object keypoijnts supervised in part from 3d reprojection error in temr sof matching 2d detected keypoints. Works of \cite{} using a pair of frames predict depth and camera motion supervised again by reprojection error. 

%Works of \cite{LSM}

Learnt stereo machines (LSM) \cite{LSM} accumulates RGB information along sequences of random camera viewpoints in  a 3D feature memory tensor, in an egomotion stabilized way, similar to our method. We compare our model to \cite{LSM} in Section \ref{sec:experiments} and show that using learning based depth estimation and early  feature unprojection  generalizes better in the presence of multiple objects that depth-unaware late unprojection,used in \cite{LSM}.  The work of \cite{3dshapenets} uses a deep generative model that given a depth map as input predicts a 3D occupancy voxel grid, and has an unprojection operation similar to the one we propose. It is trained using contrastive divergence while our model is a simple recurrent discriminative network with straightforward training. Both \cite{LSM,3dshapenets} consider the problem of single object 3D reconstruction.  Our work instead considers segmentation,  classification and 3D reconstruction of multiple objects  in clutter. %, in addition to 3d reconstructing them. 

%Simultaneous Localization And Mapping (SLAM) geometric methods have shown impressive results on estimating camera pose and 3D point clouds from monocular, stereo, or RGB-D video sequences \cite{schoeps14ismar,kerl13iros} using alternate optimization over camera poses and the 3D scene pointcloud. 

Our work produces a geometrically consistent 3D feature map of the scene using learned depth and egomotion information. Purely geometric approaches, such as  Simultaneous Localization and Mapping methods \cite{schoeps14ismar,kerl13iros} also build a 3D map of the scene while estimating the motion of the observer, but need to see the object all around in order to reconstruct it. Our work at each time step  fills missing views from experience, and improves the more views it accumulates, thus optimally combining learning and geometry. % Moreover, it detects and segments the objects, that it, it recovers semantics aided by geometrically consistent localization and  mapping.
%all around++

%camera estimation and depth estimation. 
%SE3-Nets~\cite{SE3-Nets} take as input a actuation force and a 3D point cloud to forecast a set of 3D rigid object motions (3D rotations and translations) and corresponding pixel motion masks under a static camera assumption; and their model is supervised using ground-truth 3D optical flow recorded from vicon. 
%Differentiable warping~\cite{stn,DBLP:journals/corr/PatrauceanHC15} and backpropable camera projection \cite{yan2016perspective,interpreter} have been used to  learn 3D camera motion \cite{tinghuisfm} and joint 3D camera and 3D object motion \cite{sfmnet} in an  end-to-end self-supervised fashion,  minimizing a photometric loss. 
%Garg et al.~\cite{garg2016unsupervised}given a stereo image pair with known baseline learns a monocular depth predictor, supervised by photometric error. 
%The work of \cite{handa2016gvnn} contributed a  deep learning library with many geometric operations including a back-propable camera projection layer, similar to the one used in Yan et al.~\cite{yan2016perspective} and Wu et al.~\cite{interpreter}'s cameras, as well as Garg et al.'s depth CNN~\cite{garg2016unsupervised}. 
%Our work uses differentiable camera matrices and 

\paragraph{Structured Memory}

MapNet \cite{henriques2018mapnet} aggregates visual information over time in a geometrically consistent way into a 2D birdview feature tensor, instead of a 3D one, as our method. Their task is navigation, while we attempt object detection, segmentation and labelling. 
%Since their task is localization, a 2D map is sufficient. However, since we attempt to accurately segment and reconstruct objects in 3D, we must also aggregate information in 3D. 
%While MapNet builds an allocentric representation of the environment for navigation, we use an egocentric representation and reconstruct the scene relative to the frame of the agent. \todo{this may be incorrect}

IQA \cite{DBLP:journals/corr/abs-1712-03316} u ses a similar top-down memory for interactive question answering. Like our model, their memory stores rich semantic information. One difference in our models it that IQA detects objects from single frames and accumulates detections using their memory whereas we detect objects from our memory. If an object is too heavily occluded in order to be detected by any single view, yet its existence can be inferred given the joint information from all views, then object detection from our 3D memory may succeed.

Neural Map \cite{DBLP:journals/corr/ParisottoS17} builds a 2D overhead memory in reinforcement learning environments in order to solve maze navigation tasks. 
